Bayesian Updating and Sequential Testing: Overcoming Inferential Limitations of Screening Tests

Bayes' Theorem confers inherent limitations on the accuracy of screening tests as a function of disease prevalence. We have shown in previous work that a testing system can tolerate significant drops in prevalence, up until a certain well-defined point known as the $prevalence$ $threshold$, below which the reliability of a positive screening test drops precipitously. Herein, we establish a mathematical model to determine whether sequential testing overcomes the aforementioned Bayesian limitations and thus improves the reliability of screening tests. We show that for a desired positive predictive value of $\rho$ that approaches $k$, the number of positive test iterations $n_i$ needed is: $ n_i =\lim_{\rho \to k}\left\lceil\frac{ln\left[\frac{\rho(\phi-1)}{\phi(\rho-1)}\right]}{ln\left[\frac{a}{1-b}\right]}\right\rceil$ where $n_i$ = number of testing iterations necessary to achieve $\rho$, the desired positive predictive value, a = sensitivity, b = specificity, $\phi$ = disease prevalence and $k$ = constant. Based on the aforementioned derivation, we provide reference tables for the number of test iterations needed to obtain a $\rho(\phi)$ of 50, 75, 95 and 99$\%$ as a function of various levels of sensitivity, specificity and disease prevalence.

==> bibliography.tex <==
@article{balayla2020prevalence,
  title={Prevalence Threshold and the Geometry of Screening Curves},
  author={Balayla, Jacques},
  journal={arXiv preprint arXiv:2006.00398},
  year={2020}
}

@article{balayla2020prevalence,
  title={Prevalence Threshold and Temporal Interpretation of Screening Tests: The Example of the SARS-CoV-2 (COVID-19) Pandemic},
  author={Balayla, Jacques and Lasry, Ariane and Gil, Yaron and Volodarsky-Perel, Alexander},
  journal={medRxiv},
  year={2020},
  publisher={Cold Spring Harbor Laboratory Press}
}

@article{moons1997limitations,
  title={Limitations of sensitivity, specificity, likelihood ratio, and Bayes' theorem in assessing diagnostic probabilities: a clinical example},
  author={Moons, Karel GM and van Es, Gerrit-Anne and Deckers, Jaap W and Habbema, J Dik F and Grobbee, Diederick E},
  journal={Epidemiology},
  pages={12--17},
  year={1997},
  publisher={JSTOR}
}

@article{woloshin2020false,
  title={False Negative Tests for SARS-CoV-2 Infection—Challenges and Implications},
  author={Woloshin, Steven and Patel, Neeraj and Kesselheim, Aaron S},
  journal={New England Journal of Medicine},
  year={2020},
  publisher={Mass Medical Soc}
}

@article{grimes2002uses,
  title={Uses and abuses of screening tests},
  author={Grimes, David A and Schulz, Kenneth F},
  journal={The Lancet},
  volume={359},
  number={9309},
  pages={881--884},
  year={2002},
  publisher={Elsevier}
}

@article{weisstein2002ceiling,
  title={Ceiling Function},
  author={Weisstein, Eric W},
  journal={https://mathworld. wolfram. com/},
  year={2002},
  publisher={Wolfram Research, Inc.}
}

@article{hall1967clinical,
  title={The clinical application of  Bayes' Theorem},
  author={Hall, GH},
  journal={The Lancet},
  volume={290},
  number={7515},
  pages={555--557},
  year={1967},
  publisher={Elsevier}
}

@incollection{simon1990sensitivity,
  title={Sensitivity, specificity, and predictive value},
  author={Simon, David and Boring III, John R},
  booktitle={Clinical Methods: The History, Physical, and Laboratory Examinations. 3rd edition},
  year={1990},
  publisher={Butterworths}
}

@misc{lutgendorf201699,
  title={Why 99\% may not be as good as you think it is: limitations of screening for rare diseases},
  author={Lutgendorf, Monica A and Stoll, Katie A},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{rouder2018teaching,
  title={Teaching Bayes’ theorem: Strength of evidence as predictive accuracy},
  author={Rouder, Jeffrey N and Morey, Richard D},
  journal={The American Statistician},
  year={2018},
  publisher={Taylor \& Francis}
}

@inproceedings{dezert2018total,
  title={Total belief theorem and generalized Bayes' theorem},
  author={Dezert, Jean and Tchamova, Albena and Han, Deqiang},
  booktitle={2018 21st International Conference on Information Fusion (FUSION)},
  pages={1040--1047},
  year={2018},
  organization={IEEE}
}

@article{mcgee2002simplifying,
  title={Simplifying likelihood ratios},
  author={McGee, Steven},
  journal={Journal of general internal medicine},
  volume={17},
  number={8},
  pages={647--650},
  year={2002},
  publisher={Springer}
}

@article{balayla2020derivation,
  title={Derivation of Generalized Equations for the Predictive Value of Sequential Screening Tests},
  author={Balayla, Jacques},
  journal={arXiv preprint arXiv:2007.13046},
  year={2020}
}
